Interpretable Semantic Textual Similarity: Finding and explaining differences between sentences

User acceptance of artificial intelligence agents might depend on their ability to explain their reasoning, which requires adding an interpretability layer that fa- cilitates users to understand their behavior. This paper focuses on adding an in- terpretable layer on top of Semantic Textual Similarity (STS), which measures the degree of semantic equivalence between two sentences. The interpretability layer is formalized as the alignment between pairs of segments across the two sentences, where the relation between the segments is labeled with a relation type and a similarity score. We present a publicly available dataset of sentence pairs annotated following the formalization. We then develop a system trained on this dataset which, given a sentence pair, explains what is similar and different, in the form of graded and typed segment alignments. When evaluated on the dataset, the system performs better than an informed baseline, showing that the dataset and task are well-defined and feasible. Most importantly, two user studies show how the system output can be used to automatically produce explanations in natural language. Users performed better when having access to the explanations, pro- viding preliminary evidence that our dataset and method to automatically produce explanations is useful in real applications.

==> STSgoldchunks.allresults.tex <==
\begin{table*}[!hbt]
\centering
\scriptsize
\begin{tabular}{lccccc|ccccc}
\hline
Run Name      & H ALI            & H TYPE            & H SCORE            & H T+S          & Rank         & I ALI         & I TYPE         & I SCORE         & I T+S      & Rank          \\ \hline
NeRoSim\_R3                 & 0.8976           & \textbf{0.6666}            & 0.8157             & \textbf{0.6426}  &    1                & 0.8834        & 0.6035         & 0.7837          & 0.5759         &    4      \\ 
NeRoSim\_R2                 & 0.8972           & 0.6558            & \textbf{0.8263}             & 0.6401  &    2                & 0.8800        & 0.5854         & 0.7818          & 0.5619           &     6   \\ 
NeRoSim\_R1                 & \textbf{0.8984}           & 0.6543            & 0.8262             & 0.6389 &    3                 & \textbf{0.8870}        & \textbf{0.6143}         & 0.7877          & 0.5841     &    2          \\ 
UMDuluth\_BlueTeam\_1       & 0.8861           & 0.5962            & 0.7960             & 0.5887    &       4         & 0.8853        & 0.5842         & 0.7932          & 0.5729        & 5        \\ 
UMDuluth\_BlueTeam\_2       & 0.8861           & 0.5962            & 0.7968             & 0.5883    &       5           & 0.8853        & 0.6095         & \textbf{0.7968}          & \textbf{0.5964}         &    1      \\ 
UMDuluth\_BlueTeam\_3       & 0.8861           & 0.5900            & 0.7980             & 0.5834    &       6     & 0.8853        & 0.5964         & 0.7909          & 0.5822            & 3    \\ 
SimCompass\_prefix          & 0.8360           & 0.5834            & 0.7474             & 0.5338    &       8          & 0.8361        & 0.4708         & 0.7269          & 0.4157        &   12        \\ 
SimCompass\_word2vec        & 0.8716           & 0.5806            & 0.7654             & 0.5253     &      9         & 0.8624        & 0.4599         & 0.7405          & 0.4017        &     13    \\ 
SimCompass\_combined        & 0.8710           & 0.5813            & 0.7651             & 0.5239     &      10         & 0.8490        & 0.4555         & 0.7294          & 0.3965            &   14 \\ 
ExBThemis\_avgScorer        & 0.8146           & 0.4943            & 0.7171             & 0.4885    &       11           & 0.8057        & 0.4413         & 0.6992          & 0.4246            &  11     \\ 
ExBThemis\_mostFreqScorer   & 0.8146           & 0.4943            & 0.7140             & 0.4884     &       12        & 0.8057        & 0.4413         & 0.7007          & 0.4296        &    9     \\ 
ExBThemis\_regressionScorer & 0.8146           & 0.4943            & 0.7158             & 0.4883     &       13        & 0.8052        & 0.4406         & 0.6989          & 0.4288        &      10   \\  
FCICU\_Run1                 & 0.8455           & 0.4480            & 0.7160             & 0.4325    &         14         & 0.8457        & 0.4740         & 0.7273          & 0.4482        &    7       \\ 
+RTM-DCU\_1stIBM2Alignment  & 0.4914           & 0.3712            & 0.4550             & 0.3712    &         15         & 0.3540        & 0.2283         & 0.3187          & 0.2282        &     15   \\ 
$*$UBC\_RUN2                  & 0.8991           & 0.6402            & 0.8211             & 0.6185  &           -        & 0.8846        & 0.6557         & 0.8085          & 0.6159     &    -        \\ 
$*$UBC\_RUN1                  & 0.8991           & 0.5882            & 0.8031             & 0.5882  & -                & 0.8846        & 0.4749         & 0.7709          & 0.4746        & -      \\ \hline
BASELINE                    & 0.8448           & 0.5556            & 0.7551             & 0.5556      &    7         & 0.8388        & 0.4328         & 0.7210          & 0.4326            &  8     \\ \hline
\end{tabular}
\caption{ \label{STS2c_gschunk_table} STS interpretable test results for the gold chunks scenario. Best results have been marked in bold. 'H' stands for Headlines data set and 'I' stands for Images data set.
$+$ symbol denotes resubmissions and $*$ symbol denotes task organizers.}
\end{table*}

==> STSsyschunks.allresults.tex <==
\begin{table*}[!hbt]
\centering
\scriptsize
\begin{tabular}{lccccc|ccccc}
\hline
Run Name         & H ALI            & H TYPE            & H SCORE            & H T+S       & Rank            & I ALI         & I TYPE         & I SCORE        & I T+S         & Rank    \\ \hline
UMDuluth\_BlueTeam\_3       & \textbf{0.7820}           & \textbf{0.5154}   & \textbf{0.7024}             & \textbf{0.5098}           &    1        & \textbf{0.8336}        & 0.5605         & 0.7456   & 0.5473                &    2\\ 
UMDuluth\_BlueTeam\_2       & \textbf{0.7820}           & 0.5109            & 0.6986             & 0.5049        &    2   &\textbf{ 0.8336}        & \textbf{0.5759}         & \textbf{0.7511}  & \textbf{0.5634}   &    1             \\ 
UMDuluth\_BlueTeam\_1       & \textbf{0.7820}           & 0.5058            & 0.6968             & 0.5004       &    3            & \textbf{0.8336}        & 0.5529         & 0.7498          & 0.5431         &    3       \\ 
ExBThemis\_avgScorer        & 0.7032           & 0.4331            & 0.6224             & 0.4290        & 5          & 0.6966        & 0.3970         & 0.6068          & 0.3806         & 6      \\ 
ExBThemis\_mostFreqScorer   & 0.7032           & 0.4331            & 0.6200             & 0.4288         &      6        & 0.6966        & 0.3970         & 0.6106          & 0.3870          &    4      \\ 
ExBThemis\_regressionScorer & 0.7032           & 0.4331            & 0.6209             & 0.4284      & 7            & 0.6966        & 0.3970         & 0.6092          & 0.3867     & 5         \\ 
SimCompass\_word2vec        & 0.6461           & 0.4334            & 0.5619             & 0.3878          & 8            & 0.5428        & 0.2831         & 0.4561          & 0.2427        &     8  \\
SimCompass\_prefix          & 0.6310           & 0.4284            & 0.5526             & 0.3872        &    9       & -        & -         & -          & -           & -    \\ 
SimCompass\_combined        & 0.6467           & 0.4333            & 0.5636             & 0.3870           &  10      & 0.5433        & 0.2854         & 0.4545          & 0.2421            & 9   \\ 
+RTM-DCU\_1stIBM2Alignment  & 0.4914           & 0.3712            & 0.4550             & 0.3712           &    11        & 0.3540        & 0.2283         & 0.3187          & 0.2282        &  10          \\ 
$*$UBC\_RUN2                  & 0.7709           & 0.4865            & 0.7014             & 0.4705         &    -          & 0.8388        & 0.6019         & 0.7634          & 0.5643     &    -        \\ 
$*$UBC\_RUN1                  & 0.7709           & 0.5019            & 0.6892             & 0.5019      &   -        & 0.8388        & 0.4450         & 0.7280          & 0.4447         & -    \\ \hline
BASELINE                    & 0.6701           & 0.4571            & 0.6066             & 0.4571       &    4            & 0.7060        & 0.3696         & 0.6092          & 0.3693        &    7        \\ \hline
\end{tabular}
\caption{ \label{STS2c_syschunk_table} STS interpretable test results for the system chunks scenario. Best results have been marked in bold. 'H' stands for Headlines data set and 'I' stands for Images data set.
$+$ symbol denotes resubmissions and $*$ symbol denotes task organizers.}
\end{table*}

==> analysisanddiscussion.tex <==
\section{Analysis and discussion}
\label{AnalysisDiscussion}

Given the setup of STS tasks to date, this year we wanted to shift focus and gauge the ability of participating systems to explain why two sentences may be related or unrelated, by supplementing the similarity score with an explanatory layer.
As a first step in this direction, given a pair of sentences, systems need to align the chunks across both sentences, and, also, for each alignment classify the type of relation and provide the corresponding similarity score.

On the overall, the interpretable subtask has introduced a new task where systems add a explanatory layer, in the form of alignments between text segments and explicitly  annotate the kind of relation and its score. 
It resulted on being a challenging new task that attracted the participation of seven teams (see section \ref{Test results}).

The pilot presents two scenarios:
the system chunks scenario and the gold standard chunks scenario.
In the first scenario, given a pair of sentences participants have to identify the composing chunks, and then align them.
After that, they must assign a relatedness tag and a similarity score to each alignment.
In the second scenario, on the contrary, participants are provided with gold standard chunks.



\todo{Add more on discussion}


==> interpretable_development_resultTable.tex <==
\begin{table}[!hbt]
\centering
\begin{tabular}{lcccc}
\hline
\textbf{I GS}     & \textbf{Ali} & \textbf{Type} & \textbf{Score} & \textbf{Type + Score} \\ \hline
Run1                   & 0.8942          & 0.5115           & 0.7776            & 0.5115                \\
Run2                   & 0.8942          & 0.7408           & 0.8175            & 0.6934                \\ \hline
\textbf{I SYS}    & \textbf{Ali} & \textbf{Type} & \textbf{Score} & \textbf{Type + Score} \\ \hline
Run1                   & 0.8379          & 0.4734           & 0.7271            & 0.4734                \\ 
Run2                   & 0.8379          & 0.6499           & 0.7627            & 0.6106                \\ \hline
\textbf{H GS}  & \textbf{Ali} & \textbf{Type} & \textbf{Score} & \textbf{Type + Score} \\ \hline
Run1                   & 0.8920          & 0.5740           & 0.7869            & 0.5738                \\ 
Run2                   & 0.8920          & 0.6908           & 0.8133            & 0.6544                \\ \hline
\textbf{H SYS} & \textbf{Ali} & \textbf{Type} & \textbf{Score} & \textbf{Type + Score} \\ \hline
Run1                   & 0.7650          & 0.4808           & 0.6707            & 0.4808                \\ 
Run2                   & 0.7650          & 0.5210           & 0.6862            & 0.4902                \\ \hline
\end{tabular}
\caption{\label{interpretable_development_resultTable} Development results for both datasets in the two scenarios. 'I' stands for the images dataset, and 'H' stands for the headlines dataset.}
\end{table}


==> interpretable_test_resultTable.tex <==
\begin{table}[!hbt]
\begin{tabular}{lcccc}
\hline
\textbf{I GS}  & \textbf{Ali} & \textbf{Type} & \textbf{Score} & \scriptsize\textbf{{Type + Score}} \\ \hline
Baseline        & 0.8388       & 0.4328        & 0.721          & 0.4326             \\
Run1            & 0.8846       & 0.4749        & 0.7709         & 0.4746             \\
Run2            & 0.8846       & 0.6557        & 0.8085         & 0.6159             \\
MAX Par         & 0.887        & 0.6143        & 0.7968         & 0.5964             \\
AVG Par         & 0.8193       & 0.5004        & 0.7197         & 0.4748             \\ \hline
\textbf{I SYS} & \textbf{Ali} & \textbf{Type} & \textbf{Score} & \scriptsize\textbf{{Type + Score}} \\ \hline
Baseline        & 0.706        & 0.3696        & 0.6092         & 0.3693             \\ 
Run1            & 0.8388       & 0.445         & 0.728          & 0.4447             \\ 
Run2            & 0.8388       & 0.6019        & 0.7634         & 0.5643             \\ 
MAX Par         & 0.8336       & 0.5759        & 0.7511         & 0.5634             \\
AVG Par         & 0.67         & 0.4086        & 0.5892         & 0.3912             \\\hline
\textbf{H GS}  & \textbf{Ali} & \textbf{Type} & \textbf{Score} & \scriptsize\textbf{{Type + Score}} \\ \hline
Baseline        & 0.8448       & 0.5556        & 0.7551         & 0.5556             \\ 
Run1            & 0.8991       & 0.5882        & 0.8031         & 0.5882             \\ 
Run2            & 0.8991       & 0.6402        & 0.8211         & 0.6185             \\ 
MAX Par         & 0.8984       & 0.6666        & 0.8263         & 0.6426             \\ 
AVG Par         & 0.8365       & 0.5576        & 0.7468         & 0.5381             \\ \hline
\textbf{H SYS}  & \textbf{Ali} & \textbf{Type} & \textbf{Score} & \scriptsize\textbf{{Type + Score}} \\ \hline
Baseline        & 0.6701       & 0.4571        & 0.6066         & 0.4571             \\ 
Run1            & 0.7709       & 0.5019        & 0.6892         & 0.5019             \\ 
Run2            & 0.7709       & 0.4865        & 0.7014         & 0.4705             \\ 
MAX Par         & 0.782        & 0.5154        & 0.7024         & 0.5098             \\ 
AVG Par         & 0.6870       & 0.4498        & 0.6094         & 0.4335             \\ \hline
\end{tabular}
\caption{\label{interpretable_test_resultTable}Test results for both datasets in the two scenarios.
’I’ stands for the images dataset, ’H’ stands for the headlines dataset and 'Par' stands for participants.}
\end{table}

